Subfactors of index less than 5, part 4: vines

We eliminate 38 infinite families of possible principal graphs as part of the classification of subfactors up to index 5. A number-theoretic result of Calegari-Morrison-Snyder, generalizing Asaeda-Yasuda, reduces each infinite family to a finite number of cases. We provide algorithms for computing the effective constants that are required for this result, and we obtain 28 possible principal graphs. The Ostrik d-number test and an algebraic integer test reduce this list to 7 graphs in the index range (4,5) which actually occur as principal graphs.

==> documentclasshack.tex <==
%auto-ignore
%%%%%% a hack to make the documentclass name available later %%%
% Thanks to Morten Høgholm. I stole this code from 
% http://groups.google.com/group/comp.text.tex/msg/142306cc7f8acdac
\let\LaTeXdocumentclass\documentclass
\renewcommand*\documentclass[2][]{%
   \newcommand*\ClassName{#2}% for later use
   \LaTeXdocumentclass[#1]{#2}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

